Style Outweighs Substance: Failure Modes of LLM Judges in Alignment Benchmarking

The release of ChatGPT in November 2022 sparked an explosion of interest in post-training and an avalanche of new preference optimization (PO) methods. These methods claim superior alignment by virtue of better correspondence with human pairwise preferences, often measured by LLM-judges. In this work, we attempt to answer the following question -- do LLM-judge preferences translate to progress on other, more concrete metrics for alignment, and if not, why not? We define a concrete metric for alignment, and introduce SOS-Bench (Substance Outweighs Style Benchmark), which is to the best of our knowledge the largest standardized, reproducible LLM meta-benchmark to date. We find that (1) LLM-judge preferences do not correlate with concrete measures of safety, world knowledge, and instruction following; (2) LLM-judges have powerful implicit biases, prioritizing style over factuality and safety; and (3) the supervised fine-tuning (SFT) stage of post-training, and not the PO stage, has the greatest impact on alignment, with data scaling and prompt diversity as the driving factors. Our codebase and complete results can be found at https://github.com/penfever/sos-bench.

==> tables/criteria-weighting.tex <==
\begin{table}[h]
\caption{\textbf{Judges implicitly \rev{reweight explicit} criteria.} When asked to render an overall judgment using a set of explicit criteria, models will implicitly prefer some of those criteria to others. We report the LLM's overall judgment as Arena-Hard Score, alongside independent LLM judgments of five key factors in the response. \rev{When GPT-4o-mini is the judge,} style and completeness are the strongest predictors of overall score; correctness and safety are considerably weaker, and conciseness is contra-indicated.}
\vspace{.3cm}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lllllll@{}}
\toprule
\textbf{Method} & \textbf{Arena-Hard Score} & \textbf{Completeness} & \textbf{Correctness} & \textbf{Safety} & \textbf{Conciseness} & \textbf{Style} \\ \midrule
Magpie+DPO     & 67.76 & 73.88 & 54.43 & 50.95 & 17.02 & 72.79 \\
GPT-4-0314                       & 50.00 & 50.00 & 50.00 & 50.00 & 50.00 & 50.00 \\
Meta-Llama-3-8B-Instruct         & 43.98 & 48.45 & 45.27 & 49.65 & 27.56 & 48.59 \\
Magpie & 40.81 & 46.65 & 44.21 & 49.60 & 28.19 & 47.15 \\
Tulu2+DPO & 38.36 & 44.00 & 43.74 & 49.40 & 28.39 & 44.55 \\
GPT-4-0613 & 37.68 & 35.53 & 44.30 & 49.15 & 64.03 & 39.05 \\
GPT-3.5-0125 & 34.36 & 30.77 & 44.46 & 49.60 & 65.50 & 36.87 \\
WildChat & 21.94 & 22.64 & 36.70 & 48.35 & 54.40 & 26.68 \\
Tulu2 & 14.15 & 14.02 & 33.83 & 48.44 & 58.22 & 17.94 \\
Bagel & 08.41 & 09.21 & 28.47 & 47.47 & 56.25 & 11.95 \\
Meta-Llama-3-8B & 00.44 & 00.67 & 02.66 & 25.30 & 08.80 & 00.80 \\
OPT-125m & 00.12 & 00.25 & 02.52 & 22.41 & 07.00 & 00.39 \\
\end{tabular}%
\label{tab:criteriaweighting}
}
\end{table}

==> tables/mismo-response-variations.tex <==
\centering
\begin{tcolorbox}[colback=green!5!white,colframe=green!75!black]
\begin{small}
    
\textbf{Original:}
\end{small}
\end{tcolorbox}
    \begin{tcolorbox}[colback=blue!5!white,colframe=blue!75!black]
    \begin{small}
\textbf{K:} \texttt{"Answer the question based on the task below. If the 
question cannot be answered using the information 
provided, answer with "I don't know". Task: Classify 
the column given to you into only one of these types: 
<CLASSNAMES>. Input column: <CONTEXT>. Type: "}
 \end{small}
\end{tcolorbox}
    \begin{tcolorbox}[colback=purple!5!white,colframe=purple!75!black]
    \begin{small}
\textbf{I:} \texttt{"Here is a column from a table: <CONTEXT>. 
Please select the class from that best describes the 
column, from the following options. Options: 
<CLASSNAMES> Response: "}
 \end{small}
\end{tcolorbox}
    \begin{tcolorbox}[colback=red!5!white,colframe=red!75!black]
    \begin{small}
\textbf{S:} \texttt{"Pick the column's class. Column: <CONTEXT>. 
Classes: <CLASSNAMES>. Output: "}
 \end{small}
\end{tcolorbox}
    \begin{tcolorbox}[colback=yellow!5!white,colframe=yellow!75!black]
    \begin{small}
\textbf{N:} \texttt{"Pick the column's class. I mean if you want to. It 
would be cool, I think. Anyway, give it a try, I guess? 
Here's the column itself! <CONTEXT>. And, um, 
here are some column names you could pick from ... 
<CLASSNAMES>. Ok, go ahead! "}
 \end{small}
\end{tcolorbox}
    \begin{tcolorbox}[colback=pink!5!white,colframe=pink!75!black]
    \begin{small}
    %[formatcom=\color{blue}]
\textbf{B:} \texttt{"INSTRUCTION: Select the {option | category} 
which best {describes | matches} the input. 
INPUT: <CONTEXT> OPTION: <CLASSNAMES> ANSWER:"}
 \end{small}
\end{tcolorbox}
%\vspace{-.3cm}

==> tables/two-stage-delta-v1.tex <==
\begin{table}[]
\caption{\textbf{Two-stage post-training does not improve performance on our alignment metrics.} It does, however, have a dramatic positive effect on LLM-judged benchmarks.}
\vspace{.3cm}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lllll@{}}
\toprule
\textbf{Dataset} & \textbf{DS Size (K)} & \textbf{LiveBench} & \textbf{Arena Hard} & \textbf{OpenLLM LB2} \\ \midrule
Tulu-SFT-Mix & 330 & 24.3 & 4.31 & 32.7 \\
Tulu-SFT-Mix + DPO & 390 & 19.8 & 12.4 & 32.3 \\
\textit{2-STAGE DELTA} & N/A & {\color[HTML]{FF0000} -4.5} & {\color[HTML]{0070C0} 8.09} & {\color[HTML]{FF0000} -0.4} \\
Magpie & 450 & 19.3 & 18.01 & 32.2 \\
Magpie + DPO & 510 & 15.4 & 40.81 & 33.7 \\
\textit{2-STAGE DELTA} & N/A & {\color[HTML]{FF0000} -3.9} & {\color[HTML]{0070C0} 22.8} & {\color[HTML]{0070C0} 1.5} \\
UltraChat & 200 & 18.5 & 9.2 & 33 \\
UltraChat + DPO & 260 & 16.9 & 13.81 & 31.9 \\
\textit{2-STAGE DELTA} & N/A & {\color[HTML]{FF0000} -1.6} & {\color[HTML]{0070C0} 4.61} & {\color[HTML]{FF0000} -1.1} \\
\end{tabular}%
}
\label{tab:two-stage-delta-v1}
\end{table}
